On Modal {\mu}-Calculus over Finite Graphs with Bounded Strongly Connected Components

For every positive integer k we consider the class SCCk of all finite graphs whose strongly connected components have size at most k. We show that for every k, the Modal mu-Calculus fixpoint hierarchy on SCCk collapses to the level Delta2, but not to Comp(Sigma1,Pi1) (compositions of formulas of level Sigma1 and Pi1). This contrasts with the class of all graphs, where Delta2=Comp(Sigma1,Pi1).

==> eptcsdata.tex <==
\providecommand{\event}{Angelo Montanari, Margherita Napoli, Mimmo Parente (Eds.)\\ Proceedings of GandALF 2010}
\providecommand{\volume}{25}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{55}
\providecommand{\eid}{9}

